ProtoMedX: Towards Explainable Multi-Modal Prototype Learning for Bone Health Classification

Bone health studies are crucial in medical practice for the early detection and treatment of Osteopenia and Osteoporosis. Clinicians usually make a diagnosis based on densitometry (DEXA scans) and patient history. The applications of AI in this field are ongoing research. Most successful methods rely on deep learning models that use vision alone (DEXA/X-ray imagery) and focus on prediction accuracy, while explainability is often disregarded and left to post hoc assessments of input contributions. We propose ProtoMedX, a multi-modal (multimodal) model that uses both DEXA scans of the lumbar spine and patient records. ProtoMedX's prototype-based architecture is explainable by design, which is crucial for medical applications, especially in the context of the upcoming EU AI Act, as it allows explicit analysis of model decisions, including incorrect ones. ProtoMedX demonstrates state-of-the-art performance in bone health classification while also providing explanations that can be visually understood by clinicians. Using a dataset of 4,160 real NHS patients, the proposed ProtoMedX achieves 87.58% accuracy in vision-only tasks and 89.8% in its multi-modal variant, both surpassing existing published methods.

==> sec/2_relatedWork-o.tex <==
\section{Background and Related Work}
\subsection{Bone Health}
As we age, we naturally lose bone mass. This happens to some patients at a faster rate than others, which can result in osteoporosis. Osteoporosis is a bone disease that results in an increased risk of a fragility fracture, which occurs following a fall from standing height or less. Osteoporosis affects both men and women but is most prevalent in post-menopausal women due to reduced oestrogen, with 1 in 2 women affected by the age of 80  \cite{iof_epidemiology_fragility_fractures_2025}. While it is not currently possible to completely recover bone after significant degradation, it is possible to reduce further bone loss, and the impact, through lifestyle and/or pharmaceutical interventions if detected early enough. There are several clinical tools available to assess fracture risk, including FRAX® \cite{kanis2025frax}. FRAX® calculates a patient's probability of suffering from a hip fracture caused by osteoporosis within 10 years, as well as providing advice as to whether a patient should seek a bone densitometry scan produced by a DEXA machine \cite{nogg2024manual}. The DEXA machine uses a low dose of X-Rays to measure bone mineral density and provide a T-Score. The T-Score indicates the number of standard deviations away a patient is from a young, healthy population and provides the diagnostic definition of osteoporosis, according to WHO criteria of normal bone health, osteopenia, or osteoporosis, using the following thresholds \cite{ros2025dxa}: normal (T-score above $-1.0$), osteopenia (T-score between $-1.0$ and $-2.5$), or osteoporosis (T-score below $-2.5$) \cite{ros2025dxa}.

Due to data constraints, we were limited to use lumbar spine scans, but DEXA scans are also commonly performed on hips, forearms and whole body scans.

% NEEDS A FULL REWRITE AFTER FACTS ARE FULLY THERE
\subsection{Dataset Availability}
Within the tabular data modality, early and current research often rely on relatively small datasets, typically in the range of hundreds of samples~\cite{Rae1999ANN_Osteoporosis},or moderately larger datasets (1,000–10,000 samples) that suffer from limited diversity. For example~\cite{luan2025application} employed a sample of 6,672 patients from the NHANES dataset, restricted exclusively to individuals aged 50 and above. Where for vision tasks, datasets used in research are normally in the hundreds\cite{ZHANG2020115561,9752533,sarmadi2024comparative,sukegawa2022identification}, with images coming from different parts of the body including knees, dental images and due to data restrictions, datasets are often proprietary, limiting quality of research. One example of a publicly available dataset includes 177 lumbar DEXA scans from patients in Pakistan \cite{malik2021osteoporosis}. While our dataset is not currently publicly accessible, we support ongoing efforts to promote the sharing and accessibility of such datasets within the research community.

Most studies~\cite{9752533,ZHANG2020115561,lee2019osteoporosis} rely on data augmentation methods to solve the data imbalance problem which is standard for vision tasks but there are doubts on the transferability to real clinical practice application of models that leverage augmentation within the medical domain\cite{pattilachan2023critical,tupper2024analyzing,pohjonen2022augment}.

Our research was performed in collaboration with the NHS, which allowed us to obtain a significantly larger dataset than is common in this field. Our dataset contains 4,160 patients' lumbar spine DEXA scans and basic information from their medical records. There are 2,224 patients with normal bone health, 1,398 patients with osteopenia and 538 patients with osteoporosis. The data consists of 926 males and 3,234 females. The ages of patients in the dataset range from 20 to 110, with an average age of 74 and an interquartile range of 65 to 83. 

Our dataset contains X number of tabular features. The 11 that FRAX® operates with, along with other patient information. Although it would be beneficial to analyze other features present and other feature interactions, this is beyond the scope of this paper so for validation we only included FRAX® columns. 


\subsection{Machine Learning for Bone Health}
Machine learning approaches to bone health classification have evolved from early neural networks~\cite{Ongphiphadhanakul1997BMD_ANN, Queralto1999BoneLossANN} to modern deep learning architectures. However, fundamental limitations persist across these methods.

\textbf{Tabular-only approaches} using demographic and clinical features (age, BMI, biomarkers) achieve 73-83\% accuracy~\cite{luan2025application} but lack the rich spatial information from imaging. While blood biomarkers like alkaline phosphatase provide some information, they are not diagnostic alone.

\textbf{Vision-only methods} using CNNs and Vision Transformers on DEXA/X-ray images report 80-90\% accuracy~\cite{luan2025application, sukegawa2022identification, sarmadi2024comparative, 9752533}. However, these studies suffer from: (1) binary classification that ignores the clinically important osteopenia stage~\cite{9752533}, (2) small datasets (e.g., 117 images~\cite{9752533}) with heavy augmentation, or (3) poor three-class performance (65\%~\cite{sarmadi2024comparative}). Notably, no prior work applies ViTs to lumbar spine DEXA images specifically.

\textbf{Multi-modal fusion} shows modest improvements—\cite{sukegawa2022identification} achieved 84.5\% (vs. 83.2\% vision-only) combining dental X-rays with demographics. While this study employed binary classification, it demonstrates that the addition of tabular features in a Multi-Modal setting can provide modest accuracy gains, which is in line with our own findings.

These approaches share critical gaps: oversimplified binary classification, lack of explainability, and limited multi-modal integration, motivating our prototype-based solution that addresses all three.

% The backbones of the best results were Inveption v3 and VGG16, achieving 92.1\% and 90.5\% accuracy respectively, but on minimal data and using strong augmentation\cite{9752533}. WHERE DOES THIS PAPER GO?  (If later needed)

\begin{comment}
    \subsection{Machine Learning for Bone Health}

The application of machine learning to bone health is not new. Since the 1990s, techniques such as logistic regression and early artificial neural networks have been explored for the detection and diagnosis of osteoporosis~\cite{Ongphiphadhanakul1997BMD_ANN, Queralto1999BoneLossANN}. 

% ARE THERE NO MORE STUDIES ?
Tabular features are attractive due to their low acquisition cost, commonly including demographic information, patient history, and lifestyle variables. However, these alone are insufficient for accurate bone health prediction, as shown in [our results / Table X / prior studies – adjust based on actual source]. Consequently, higher-value but higher acquisition cost features are frequently integrated, such as outputs from DEXA scans—namely Bone Mineral Density (BMD) and T-scores—which offer direct indicators of bone health status [insert small motivating example + reference here].

Additional features may include clinical and laboratory measurements such as blood biomarkers (e.g., creatine phosphokinase, alkaline phosphatase, cholesterol, glucose, hemoglobin)~\cite{luan2025application}. [Add comment here depending on whether these are costly to obtain, outside standard guidelines, or hard to scale—e.g., “While potentially informative, these biomarkers may not be routinely collected in osteoporosis screening workflows, limiting real-world applicability.”]

Furthermore, many prior studies approach bone health classification as a binary task. Typically distinguishing between normal and low bone density. This framing oversimplifies the problem by ignoring the continuous nature of bone density variation, as well as the clinical need to differentiate among the three diagnostic categories: normal, osteopenia, and osteoporosis. This limitation is also reflected in [TSNE visualizations / confusion matrices / clinical guidelines – insert evidence or citation] 

The aforementioned studies show promising results. Ranging between 73\% in logistic regression and 83\% using standard neural networks. [Sorry please add the references again and edit this for correctness]

% VISION - X things - Y REsults - Z Backbones - (They are explainable or not, next section) 

Within the vision modality, state-of-the-art (SOTA) approaches primarily leverage Deep Neural Networks (DNNs) applied to medical imaging—commonly Dual-energy X-ray Absorptiometry (DEXA) or standard X-ray scans—with reported classification accuracies typically ranging between 80–90\%. Recent advances predominantly involve Vision Transformers (ViTs) and Convolutional Neural Networks (CNNs)~\cite{luan2025application, sukegawa2022identification, sarmadi2024comparative, 9752533}.

For example, Ref.~\cite{9752533} employed InceptionV3 for binary classification (normal vs osteoporosis) on lumbar spine DEXA images, claiming a 92.1\% accuracy. However, their methodological transparency is limited, as data splits used in experiments were not explicitly detailed. Their entire dataset consisted of only 117 images, some of which were excluded due to the binary-label constraint, and the study relied heavily on data augmentation, raising questions regarding its generalizability.

In contrast,~\cite{sarmadi2024comparative} utilized Vision Transformers (ViTs) for a more clinically relevant three-class classification task (normal, osteopenia, osteoporosis) based on knee DEXA scans, reporting a maximum accuracy of 65\%. This study explicitly addressed dataset imbalance—common in clinical data—and intentionally avoided augmentation, making it a realistic baseline for our own vision modality experiments. Additionally, their findings suggest potential advantages of transformer-based approaches for this task, further supported by our comparative results presented in Section\ref{sec:results?}, Table~\ref{tab:models}. To the best of our knowledge, no prior studies have employed ViTs specifically on lumbar spine DEXA images.

Further research into heterogeneous data classification, which combines medical imaging with basic patient demographic information, has shown promising results. The highest reported accuracy in existing literature~\cite{sukegawa2022identification} was 84.5\% when integrating dental X-ray images (EfficientNet-B7) with demographic features (age, sex, BMI), compared to 83.2\% when only images were considered. This suggests a modest but meaningful improvement through additional tabular data, aligning with our own findings. However, this prior study differs significantly from ours, as it employed a binary osteoporosis/non-osteoporosis classification on dental imagery rather than the clinically oriented three-class task on lumbar spine imagery addressed in this work. [clarify explicitly if dental imaging inherently yields significantly different results or has different clinical relevance compared to lumbar spine imaging.]


\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Interpretable AI for Medical Imaging} % Change the title?
Clinical deployment demands models that are able to explain their reasoning, not just achieve high accuracy. Post-hoc methods like GradCAM \cite{selvaraju2019grad}, SHAP \cite{NIPS2017_7062}, and saliency maps \cite{zeiler2014visualizing} approximate model behavior after training but lack fidelity and have the capability of being misleading. They provide rationalizations rather than true model reasoning \cite{rudin2019stop,hooshyar2024problems,krishna2022disagreement,witzel2024explainable,gosiewska2020donottrust}. This disconnect is particularly problematic in medical contexts where understanding the decision process guides treatment.

\paragraph{Prototype-based Models:} Prototype learning offers inherent explainability by comparing inputs to learned exemplars. ProtoPNet \cite{Chen2019} pioneered this approach for images followed shortly by xDNN approach \textbf{{add reference Anglelov and Soares, 2020}}, enabling case-based reasoning ("this looks like prototype X"). However, ProtoPNet suffers from three limitations: (1) vision-only architecture makes the framework incompatible with clinical data, (2) reliance on localized patches that can highlight misleading regions [ADD APPENDIX REFERENCE TO OUR OWN TEST OR SOME OTHER PROOF], and (3) post-hoc similarity heatmaps rather than supervised prototype learning \cite{tegerdine_willard_triplett_tang_2023}. xDNN also suffers from (1).
\begin{figure}[]
    \centering

    % Top row group
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img0.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth,clip,trim=0 100 0 0]{ICCV2025-Author-Kit/img/prototype-img14.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img7.png}
        \end{subfigure}
        \caption{Prototypes provided}
    \end{subfigure}

    \vspace{1em}

    % Bottom row group
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img-original_with_self_act0.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img-original_with_self_act14.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img-original_with_self_act7.png}
        \end{subfigure}
        \caption{Heatmaps provided}
    \end{subfigure}

    \caption{These provided ProtoPNet prototypes for osteoporosis cases are ok, with the best being the rightmost. The heatmaps offer little assistance for the first two.}
    \label{fig:full_grid}
\end{figure}


\begin{figure}[]
    \centering
    % Top row group
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img4.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img8.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img12.png}
        \end{subfigure}
        \caption{Prototpyes provided}
    \end{subfigure}

    \vspace{1em}

    % Bottom row group
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img-original_with_self_act4.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img-original_with_self_act8.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\columnwidth}
            \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/img/prototype-img-original_with_self_act12.png}
        \end{subfigure}
        \caption{Heatmaps provided}
    \end{subfigure}

    \caption{These provided ProtoPNet prototypes and heatmaps for osteoporosis cases are NOT ok, with all of them focusing on areas outside of the bone.}
    \label{fig:full_grid}
\end{figure}


To the best of our knowledge, no prior work applies prototype-based learning to bone health classification. \textbf{ProtoMedX} addresses this gap by extending prototype reasoning to multi-modal inputs (imaging + clinical data) while learning full-image prototypes that provide clearer clinical interpretation than ambiguous local patches. This design aligns with the way clinicians reason, comparing patients to archetypal cases rather than analyzing isolated image regions.

\begin{comment}
    \subsection{Explainable Methods for Bone Health} % RETHINK TITLE

Model accuracy with limited data is only part of the challenge. Real clinical applications demand models capable of revealing their decision-making rationale, often referred to in ML literature as explainability or interpretability, since transparency and trust become critical in high-stakes medical settings unless performance is exhaustively validated—something commonly achieved in robotics domains but not yet standard in healthcare [CITATION NEEDED FOR ROBOTICS CLAIM].

Popular post-hoc explainability methods, applied after model training, include saliency maps \cite{zeiler2014visualizing}, activation maximization \cite{erhan2009visualizing}, SHAP \cite{NIPS2017_7062}, Grad-CAM \cite{selvaraju2019grad}, and perturbation-based approaches \cite{ivanovs2021perturbation}. These methods attempt to approximate model reasoning after the fact.

However, post-hoc techniques often fall short in faithfulness. They offer only indirect explanations rather than unveiling the model’s true decision logic [CITATION NEEDED]. They are not tightly coupled with the model's internal computations, which raises questions about their reliability in clinical use [CITATION NEEDED]. The recent XAI literature highlights this limitation and calls for self-explainable or explainable by design models, which embed interpretability/explainability directly into the architecture, rather than relying on peripheral explanation tools [CITATION NEEDED]. In medical imaging contexts, regulatory and clinical standards—whether applied to stethoscopes, X-ray devices, or DEXA scanners—expect devices to be understandable by design, reinforcing the need for inherently interpretable AI. In this work, we push forward this agenda by focusing on prototype-based, inherently explainable/Interpretable models for bone-health prediction. A novel direction in this domain.


\paragraph{Prototype-based Models for Bone Health:} To the best of our knowledge there have been no available publications exploring the use of prototype=based models towards explainable Bone Health classification.

Prototype-based models use representative examples (prototypes) that capture prototypical features of each class. Unlike post-hoc methods, which attempt to justify model decisions after inference, prototype-based models compare new inputs directly to learned primitives during decision-making. This fosters interpretability/explainability: clinicians can see which known cases the model references (“input X is similar to prototype Y”) and understand the decision boundaries visually.

A prime example is ProtoPNet \cite{Chen2019}, which learns prototypes during training and then reasons by comparing them to image regions. However, ProtoPNet is limited to single-modality vision data, making it incompatible with multi-modal inputs. In contrast, our proposed ProtoMedX extends this concept to support multi-modal prototype-based reasoning, integrating both images and tabular patient data.

That said, prototype-based models like ProtoPNet still rely on post-hoc heatmap visualizations derived from similarity scores—not explicitly supervised during training; hence their interpretability may lack clarity and robustness, especially in datasets that lack fine-grained region annotations \cite{tegerdine_willard_triplett_tang_2023}. As dataset size grows, tight localization becomes even more challenging and resource-intensive to label.

In our early experiments, we observed that ProtoPNet often highlighted misleading prototypes in X-ray queries [CAN WE DEMONSTRATE THIS, PROBABLY APPENDIX], which risked confusion for clinicians. Although we are not yet solving this granularity issue, we argue that presenting full-image prototypes, rather than ambiguous localized regions, offers a more practical and trustworthy interface for clinicians—while still encouraging future work to refine prototype localization.


% In 2023, researchers compared ProtoPNet to ResNet18 and achieved a higher accuracy using ProtoPNet (68.5\% compared to 65.4\%)\cite{carloni2022applicability}.

\end{comment}


==> sec/3_architectureAndData-o.tex <==
\section{ProtoMedX}
ProtoMedX introduces prototype-based deep learning for bone health assessment, enabling case-based reasoning and explanations that align with clinical decision-making. It learns class-representative prototypes in a unified feature space, making predictions by comparing inputs to these prototypes. Fig.~\ref{fig:architecture} illustrates the overall architecture of the proposed framework.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{img/ProtoMedX-Architecture.png}
    \caption{
        \textbf{Overview of ProtoMedX Architecture.} 
        Multi-modal prototype learning combines patient DEXA scans and clinical records via separate encoders, learns interpretable vision and tabular prototypes, and fuses them in a joint prototype space. Classification and explanations derive from prototype similarity and case retrieval, enhancing clinical interpretability.
    }
    \label{fig:protomedx_architecture}
\end{figure*}


\subsection{Feature Extraction and Encoding}
\textbf{Vision Branch:} We employ a frozen CrossViT backbone \cite{chen2021crossvit} pre-trained on ImageNet for DEXA feature extraction. CrossViT's dual-branch design captures both fine-grained trabecular patterns and global spinal morphology, critical for osteoporosis assessment. Among tested backbones, CrossViT achieved superior standalone performance:



The frozen backbone outputs $\mathbf{f}^{\text{img}}\in\mathbb{R}^{1151}$, which is fed to a projection MLP
$(1151\!\rightarrow\!512\!\rightarrow\!256)$ with BatchNorm and $0.3$ dropout,
producing
\[
\mathbf{h}_i=\phi_i(\mathbf{f}^{\text{img}})\in\mathbb{R}^{256}.
\]

\textbf{Tabular Branch:} We encode the Clinical features as a vector $\mathbf{x}^{\text{tab}}\in\mathbb{R}^{11}$ (age, BMI, fracture history, etc.) via
\[
\mathbf{h}_t = \phi_t(\mathbf{x}^{\text{tab}}),\qquad
\phi_t:\mathbb{R}^{11}\!\rightarrow\!\mathbb{R}^{64},
\]
where $\phi_t$ is a two-layer MLP with residual connections and dropout.

\subsection{Cross-Modal Fusion}

The encoded image and tabular embeddings are first combined by a cross-modal
attention block, producing a joint representation:
\[
\mathbf{h}_{\mathrm{fused}}
      = \operatorname{CrossAtt}\bigl(\mathbf{h}_i,\mathbf{h}_t\bigr)
      \in\mathbb{R}^{256}.
\]

\vspace{4pt}
\noindent
During prototype matching we apply an adaptive, input-dependent weighting
of modality-specific similarity scores:
\[
\alpha = \sigma\!\bigl(g([\mathbf{h}_i;\mathbf{h}_t])\bigr),\qquad
\mathrm{sim}(\mathbf{z})
      = \alpha\,S_{\text{img}}(\mathbf{z})
      + (1-\alpha)\,S_{\text{tab}}(\mathbf{z}),
\]
where $g$ is a linear layer and
$S_{\text{img}},\,S_{\text{tab}}$ are cosine similarities in the image and
tabular prototype sub-spaces, respectively.
This gating strategy improved top-1 accuracy by $1.2\%$ compared with uniform
weighting.  The fused vector $\mathbf{h}_{\mathrm{fused}}$ is subsequently
fed to the prototype layer for classification.
\begin{comment}
    \subsection{Cross-Modal Fusion}

A learnable gate balances modality contributions based on input characteristics:
\begin{equation}
\alpha = \sigma(g([\mathbf{h}_i; \mathbf{h}_t])), \quad \mathbf{h}_{fused} = \alpha \mathbf{h}_i + (1-\alpha) \mathbf{h}_t
\end{equation}
where $g$ is a linear layer. Ablation study shows that this gating improves accuracy by 1.2\% over simple concatenation. The fused representation undergoes cross-attention to model inter-modal dependencies before it is passed to the prototype layer.

\end{comment}


\subsection{Prototype Learning}

ProtoMedX learns $K=6$ prototypes per class, where each prototype represents a typical patient case. This value was determined through empirical validation: $K<6$ failed to capture intra-class diversity (e.g., early vs. advanced osteoporosis), while $K>6$ introduced redundant prototypes without improving classification. We employ a dual prototype architecture maintaining separate spaces for visual ($\mathbf{p}_{c,k}^{img} \in \mathbb{R}^{128}$) and tabular ($\mathbf{p}_{c,k}^{tab} \in \mathbb{R}^{64}$) features while performing classification in the fused space. This enables modality-specific interpretation. Ablation shows that removing dual prototypes reduces accuracy by 6.5\%.

Following contrastive learning principles \cite{chen2020simple}, we optimize prototypes through a composite loss:
\begin{equation}
\mathcal{L}_{proto} = \mathcal{L}_{class} + \lambda_{sep}\mathcal{L}_{sep} + \lambda_{ctr}\mathcal{L}_{center}
\end{equation}

where $\mathcal{L}_{class}$ ensures prototypes alone can classify via softmax over cosine similarities, $\mathcal{L}_{sep}$ maintains inter-class margins using a triplet-like loss [Add triplet loss reference - Schroff et al. 2015], and $\mathcal{L}_{center}$ compacts intra-class distributions [Add center loss reference - Wen et al. 2016]. This creates well-separated clusters (Fig.~\ref{fig:tsne}) with osteoporosis prototypes clustering at low T-scores (-3.48 average).

To maintain interpretability, prototypes are periodically projected onto nearest training examples, ensuring that each represents an actual patient case rather than abstract features.

\subsection{Multi-Task Learning}

Traditional approaches inadequately exploit the fact that the bone density has a continuous nature and have notable limitations: tabular methods heavily rely on external BMD values, achieving only 45\% accuracy without them (Table~\ref{tab:tabular}); two-stage vision frameworks that first predict BMD to make the diagnosis suffer from large classification errors due to sharp clinical thresholds at T=-1 and T=-2.5 (Table~\ref{tab:BMD}); direct classification ignores continuous bone-density variations, plateauing at about 70\% accuracy, although not far from the standard cross-entropy approaches. (See Table~\ref{tab:full-experiments}).

We address these issues using multi-task learning, jointly optimizing for classification and T-score regression. This encourages the model to learn continuous bone-density representations, smooth decision boundaries, and regularize training. Formally:

\begin{equation}
\mathcal{L}_{ProtoMedX} = \mathcal{L}_{cls} + \lambda_1\mathcal{L}_{reg} + \lambda_2\mathcal{L}_{proto}
\end{equation}

where $\mathcal{L}{cls}$ handles classification, $\mathcal{L}{reg}$ predicts T-scores, and $\mathcal{L}_{proto}$ is the prototype learning loss. Including regression ($\lambda_1=0.3$) significantly improves accuracy—removing it results in a 6.7\% accuracy drop. Thus, explicitly modeling bone-density continuity substantially enhances clinical predictions which at the end are in a form of 3-class classification (Normal/ Osteopenia/Osteoporosis). 

\subsection{Clinical Explanations}

ProtoMedX provides clinically interpretable, multi-level explanations for each diagnosis (see Fig.~\ref{fig:clinical_explanations}).

\textbf{Classification Confidence:} Model confidence is derived from the weighted k-NN voting among prototypes:

\begin{equation}
\mathcal{C}=\frac{\sum_{i\in\mathcal{N}_c}e^{-d_i/\tau}}
                  {\sum_{j=1}^k   e^{-d_j/\tau}},
\end{equation}
where $\mathcal{N}_c\subseteq\{1,\dots,k\}$ are the $k$ nearest prototypes
of the predicted class $c$, $d_i$ is the Euclidean distance to prototype $i$,
and $\tau$ controls the sharpness of the weighting.

\begin{comment}
    

\begin{equation}
\mathcal{C} = \frac{\sum_{i \in \mathcal{N}_c} w_i}{\sum_{j=1}^k w_j}, \quad w_i = \exp(-d_i/\tau)
\end{equation}
where:
\begin{itemize}
    \item $\mathcal{C}$ is the confidence score representing the relative contribution of class-supporting prototypes
    \item $\mathcal{N}_c$ contains indices of the $k$ nearest prototypes that belong to the predicted class $c$
    \item $w_i = \exp(-d_i/\tau)$ is the weight of prototype $i$ based on its distance
    \item $d_i$ is the Euclidean distance between the input representation and prototype $i$ % Need to check if Euclidean or Cosine
    \item $\tau$ is the temperature parameter controlling the sharpness of the distance-based weighting (smaller $\tau$ gives sharper focus on nearest prototypes)
    \item $k$ is the total number of nearest prototypes considered in the k-NN classification
    \item The numerator sums weights of prototypes supporting the predicted class
    \item The denominator normalizes by the sum of all $k$ prototype weights
\end{itemize}
\end{comment}


High confidence (e.g. \( >90\% \)) indicates strong consensus; low confidence (e.g. \( <60\% \)) highlights borderline or uncertain cases. An advantage of the proposed ProtoMedX is the ability to analyze the decisions. It is characteristic that the confidence is quite low (48.9\%) for the decisions which turn out to be wrong while the confidence for the decisions which are correct is quite high (85.3\% on average).

\textbf{Prototype-based Reasoning:} Each decision is supported by the most similar $k$ ($k=3$) prototypes, displaying source patient ID, clinical features (T-score, age, BMI, fracture history), influence weight, and prototype representativeness. For example: “Patient matches prototype P13 (weight 0.395, T-score -2.49), representing 70 similar cases.”

\textbf{Feature-Level Analysis:} For each clinical feature $j$, we compute relative deviation from class norms  (for class c):
\begin{equation}
\delta_j = \frac{|x_j^{tab} - \mu_{c,j}|}{\max(\mu_{c,j}, 1)}
\end{equation}
Features with $\delta_j > 0.5$ (highlighted in red) signal clinically atypical values. (See Fig~\ref{explanation} 

\textbf{Voting Visualization:} Bar plots show vote distributions, helping identify borderline versus confident classifications. % Might delet if we dont find evidence in figures

\textbf{Misclassification Analysis:} First of all, the proposed ProtoedX provides confidence which is an indication of a possible misclassification as described earlier. Furthermore, for the errors, the system visualizes both predicted and true class prototypes, supporting error analysis. Most mistakes occur near diagnostic boundaries (e.g., Normal→Osteopenia). Fig. ~\ref{missclassification} shows an example % Maybe move to resutls

\subsection{Prototype-Based Classification}

During inference, ProtoMedX performs explainable classification through k-nearest neighbor search:

\begin{algorithm}[H]
\caption{ProtoMedX Inference and Explanation Generation}
\begin{algorithmic}[1]
\State \textbf{Input:} Patient $(\mathbf{x}^{img}, \mathbf{x}^{tab})$, Learned prototypes $\mathbf{P}$
\State \textbf{// Feature extraction and fusion}
\State $\mathbf{z}, \alpha \leftarrow \text{EncodeFuse}(\mathbf{x}^{img}, \mathbf{x}^{tab})$ 
\State \textbf{// k-NN classification}
\State Compute distances: $d_{c,k} = \|\mathbf{z} - \mathbf{p}_{c,k}\|_2$ for all prototypes
\State Select k=3 nearest prototypes: $\mathcal{N} = \{(c_i, k_i, d_i)\}_{i=1}^3$
\State Calculate weights: $w_i = \exp(-d_i/\tau)$, normalize to sum to 1
\State Vote: $v_c = \sum_{i: c_i=c} w_i$ for each class $c$
\State Predict: $\hat{y} = \arg\max_c v_c$
\State \textbf{// Generate clinical explanation}
\State Confidence: $\mathcal{C} = v_{\hat{y}}$ (winning vote weight)
\State Retrieve prototype metadata: patient IDs, T-scores, clinical features
\State Compute feature deviations: $\delta_j = |x_j^{tab} - \mu_{\hat{y},j}|/\max(\mu_{\hat{y},j}, 1)$
\State Flag atypical features where $\delta_j > 0.5$
\State \textbf{Return:} Class $\hat{y}$, confidence $\mathcal{C}$, similar patients $\mathcal{N}$, 
\State \quad\quad\quad modality weight $\alpha$, feature analysis $\{\delta_j\}$
\end{algorithmic}
\end{algorithm}

This approach achieves 83.9\% accuracy with k-NN classification, comparable to neural network performance (83.8\%) while providing complete interpretability.

% THIS IS GOOD BUT TOO LONG:

\begin{comment}
    \subsection{Multi-Task Learning}

While our primary objective is three-class classification (Normal/Osteopenia/Osteoporosis), we observe that existing approaches fail to leverage the continuous nature of bone density. Traditional methods fall into three problematic categories:

\begin{itemize}
\item \textbf{Tabular methods} require the addition of pre-computed BMD values from DEXA machines along with the other FRAX®, achieving only 45\% accuracy without them according to our own experiments. (See Table~\ref{tab:tabular})
\item \textbf{Two-stage approaches} first predict BMD then classify, but small regression errors cause large classification mistakes due to sharp decision boundaries at T=-1 and T=-2.5 demonstrated by our experiments (See Table~\ref{tab:BMD})
\item \textbf{Direct classification} ignores the underlying continuous distribution, plateauing at ~70\% accuracy (See Table~\ref{tab:full-experiments})
\end{itemize}

Our key insight: jointly learning T-score regression guides the model to understand bone density as a continuum rather than discrete categories. The regression task acts as an auxiliary objective that (1) Forces the model to learn representations that capture continuous bone density variations (2) Smooths decision boundaries near diagnostic thresholds (3) Provides implicit regularization preventing overfitting to discrete labels.

We exploit this through joint optimization:

\begin{equation}
\mathcal{L}_{total} = \mathcal{L}_{cls} + \lambda_1\mathcal{L}_{reg} + \lambda_2\mathcal{L}_{proto}
\end{equation}

where $\mathcal{L}_{cls}$ handles classification, $\mathcal{L}_{reg}$ provides T-score supervision, and $\mathcal{L}_{proto}$ implements the prototype learning objectives detailed above. The T-score regression ($\lambda_1=0.3$) forces understanding of bone density continuity—removing it reduces accuracy by 6.7\%, confirming that continuous supervision enhances categorical prediction.

This demonstrates that understanding the continuous nature of bone density, even imperfectly, significantly improves categorical diagnosis, the ultimate clinical objective.



\subsection{Clinical Explanations}

ProtoMedX generates multi-faceted explanations for each diagnosis, transforming opaque predictions into clinically interpretable insights. Fig.~\ref{fig:clinical_explanations} demonstrates the comprehensive explanation system across all diagnostic categories.

\textbf{Classification Confidence:} Confidence derives from the k-NN voting distribution among prototypes:
\begin{equation}
\mathcal{C} = \frac{\sum_{i \in \mathcal{N}_c} w_i}{\sum_{j=1}^k w_j}, \quad w_i = \exp(-d_i/\tau)
\end{equation}
where $\mathcal{N}_c$ contains indices of prototypes voting for predicted class $c$. High confidence (>90\%) indicates consensus, while lower values (<60\%) flag borderline cases requiring clinical review. Analysis reveals correct predictions average 85.3\% confidence versus 48.9\% for misclassifications.

\textbf{Prototype Reasoning:} Each prediction traces to k=3 most similar patient cases, providing:
- **Source patient**: Original image ID and clinical profile
- **Similarity weight** $w_i$: Quantifies influence on final prediction  
- **Clinical characteristics**: T-score, key features (age, BMI, fracture history)
- **Representativeness**: Cluster size showing how many training patients this prototype represents

Example explanation: "Patient resembles prototype P13 (weight: 0.395) from 9bacwd1yt.png - Osteopenia class, T-score: -2.49, representing 70 similar patients with average age 68.8 years and previous fracture rate 1.0."

\textbf{Feature-Level Analysis:} For each clinical feature $j$, we compute relative deviation from class norms (for class c):
\begin{equation}
\delta_j = \frac{|x_j^{tab} - \mu_{c,j}|}{\max(\mu_{c,j}, 1)}
\end{equation}
Features with $\delta_j > 0.5$ are highlighted in red (Fig.~\ref{fig:clinical_explanations}), indicating atypical values influencing classification. Common patterns include elevated age and previous fractures for younger osteoporosis patients.

\textbf{Voting Visualization:} Bar charts display the classification decision process, showing vote weights across all classes. This reveals borderline cases (near-equal votes) and confident classifications (dominant single class).

\textbf{Misclassification Analysis:} For incorrect predictions, the system shows both predicted and true class prototypes, enabling error analysis. Common confusion patterns include Normal→Osteopenia (7 cases) and Osteoporosis→Osteopenia (5 cases), typically occurring at diagnostic boundaries.



\end{comment}





\begin{comment}

\section{ProtoMedX: Multi-Modal Prototype-Based Framework}

ProtoMedX predicts bone health classification labels $y \in \{0, 1, 2\}$ corresponding to Normal, Osteopenia, and Osteoporosis, respectively. The architecture consists of: (1) modality-specific encoders, (2) attention-based fusion, (3) prototype layer learning class representatives, and (4) multi-task heads for classification and T-score regression. Classification is performed by finding the class whose prototypes have maximum similarity to the input representation [AS DEPICTED IN FIG. X].

\subsection{Feature Extraction}

\textbf{Vision Branch:} We employ a frozen CrossViT backbone \cite{Chen2021} for extracting visual features from DEXA lumbar spine scans. CrossViT was selected as it achieved the highest standalone performance across our experiments


%% How do we fairly represent this, when these figures are from the previous, incorrect, T-Scores?
\begin{table}[ht]
\centering
\label{tab:vision_backbone_comparison}
\begin{tabular}{lccc}
\toprule
\textbf{Backbone} & \textbf{Accuracy (\%)} \\
\midrule
ResNet            & 78\\
DenseNet          & 81\\
ViT               & 83\\
DeiT              & 83\\
\textbf{CrossViT} & \textbf{85} \\
\bottomrule
\end{tabular}
\caption{Comparison of Vision Backbone Models on standalone Bone Health classification}
\end{table}

The dual-branch multi-scale design of CrossViT is particularly suited for DEXA analysis: the fine-grained branch captures local trabecular bone patterns indicative of microarchitectural deterioration, while the coarse-grained branch models global spinal alignment and vertebral morphology - both critical factors in osteoporosis assessment \cite{chen2021crossvit}.

The frozen backbone outputs $\mathbf{f}^{img} \in \mathbb{R}^{1151}$ which undergoes dimensionality reduction:
\begin{equation}
\mathbf{h}_i = \phi_i(\mathbf{f}^{img}) \in \mathbb{R}^{256}
\end{equation}
where $\phi_i$ represents a projection network with batch normalization and dropout for regularization.

\textbf{Tabular Branch:} Clinical features $\mathbf{x}^{tab} \in \mathbb{R}^{d_{tab}}$ undergo feature-wise attention to automatically learn importance weights, motivated by the FRAX® tool which assigns different weights to risk factors \cite{kanis2025frax}:
\begin{equation}
\mathbf{w} = \sigma(\psi(\mathbf{x}^{tab})), \quad \mathbf{h}_t = \phi_t(\mathbf{x}^{tab} \odot \mathbf{w})
\end{equation}
where $\psi$ is a two-layer attention network and $\phi_t$ is the tabular encoder with residual connections.

\subsection{Joint Classification and T-Score Regression}

In clinical practice, osteoporosis diagnosis relies on Bone Mineral Density (BMD) measured by DEXA machines using dual-energy X-ray radiation. This BMD value, combined with population-based indicators, is converted to a T-score that defines diagnostic categories: Normal ($T > -1$), Osteopenia ($-2.5 < T \leq -1$), and Osteoporosis ($T \leq -2.5$).

Existing ML approaches face fundamental limitations:
\begin{itemize}
\item \textbf{Tabular-only methods} require Bone Mineral Density (BMD) values as input features, achieving poor performance without them 

% [Add Table X: showing <50\% accuracy without BMD]


\item \textbf{BMD regression approaches} first predict BMD from images, then classify. While achieving reasonable MSE for BMD prediction, the high sensitivity of class boundaries to small BMD variations leads to poor classification accuracy
% [Add Table Y: BMD regression MSE vs classification accuracy]



\item \textbf{Direct classification approaches} bypass BMD entirely but plateau around 70\% accuracy due to the continuous nature of bone deterioration
\end{itemize}

We leverage the deterministic relationship between T-score and class:
\begin{equation}
y = \begin{cases}
0 \text{ (Normal)} & \text{if } t > -1 \\
1 \text{ (Osteopenia)} & \text{if } -2.5 < t \leq -1 \\
2 \text{ (Osteoporosis)} & \text{if } t \leq -2.5
\end{cases}
\end{equation}

Both outputs are predicted from shared features:
\begin{align}
\hat{y} &= \text{softmax}(\mathbf{W}_c[\mathbf{h}_{fused}; \mathbf{l}] + \mathbf{b}_c) \\
\hat{t} &= \mathbf{w}_r^T[\mathbf{h}_{fused}; \mathbf{l}] + b_r
\end{align}

where $\mathbf{l}$ are prototype logits. The joint loss ensures consistency:
\begin{equation}
\mathcal{L}_{joint} = \mathcal{L}_{CE}(y, \hat{y}) + \lambda_{reg}\mathcal{L}_{MSE}(t, \hat{t})
\end{equation}

This formulation teaches the model to respect the continuous nature of bone health while focusing on correct classification. [Justification: Ablation study shows >10\% improvement with joint learning vs classification-only].

\subsection{Cross-Modal Fusion}

Simple concatenation treats modalities equally, but clinical features should provide context that modulates interpretation of imaging features. [Justification: In clinical practice, identical DEXA appearances require different interpretations based on patient demographics - a 70-year-old woman's "normal" differs from a 30-year-old man's].

Given visual features $\mathbf{h}_i \in \mathbb{R}^{256}$ and tabular features $\mathbf{h}_t \in \mathbb{R}^{256}$, we first project them:
\begin{align}
\mathbf{Q} &= \mathbf{h}_i\mathbf{W}_Q, \quad \mathbf{K} = \mathbf{h}_t\mathbf{W}_K, \quad \mathbf{V} = \mathbf{h}_t\mathbf{W}_V
\end{align}

Multi-head attention computes:
\begin{align}
\mathbf{A} &= \text{softmax}\left(\frac{\mathbf{Q}\mathbf{K}^T}{\sqrt{d_k}}\right) \\
\mathbf{h}_{att} &= \mathbf{A}\mathbf{V}
\end{align}

The final fused representation:
\begin{equation}
\mathbf{h}_{fused} = \text{MLP}([\mathbf{h}_i \oplus \mathbf{h}_t \oplus \mathbf{h}_{att}])
\end{equation}
where $\oplus$ denotes concatenation, $d_k=128$. [Justification: Attention visualization shows model learns clinically meaningful associations - degraded trabecular patterns trigger higher attention to age and fracture history].

\subsection{Prototype Layer}

% This first line is just wrong
Following \cite{chen2019this}, we maintain $K=3$ prototypes per class $\mathbf{P} = \{\mathbf{p}_{c,k}\}_{c=1}^{C}$. [Justification: Validation showed K=3 optimal - K=1 underfits class diversity, K>3 introduces redundancy without accuracy gain].

Each prototype $\mathbf{p}_{c,k} \in \mathbb{R}^{128}$ is initialized using k-means++ on training features of class $c$. Given fused features, we apply a refinement network:
\begin{equation}
\mathbf{z} = \text{ReLU}(\text{BN}(\mathbf{W}_{refine}\mathbf{h}_{fused} + \mathbf{b}_{refine}))
\end{equation}

Similarities are computed using complementary metrics:
\begin{equation}
s_{c,k} = \frac{\langle \bar{\mathbf{z}}, \bar{\mathbf{p}}_{c,k} \rangle}{\tau}, \quad d_{c,k} = \|\mathbf{z} - \mathbf{p}_{c,k}\|_2
\end{equation}

where $\bar{\cdot}$ denotes L2-normalization and $\tau=0.05$. [Justification: Cosine similarity handles DEXA intensity variations from patient size/machine calibration; Euclidean distance ensures absolute proximity for confident classification].

Class logits: $l_c = \max_k s_{c,k}$

\subsection{Training Objective}

The complete loss balances multiple objectives:
\begin{equation}
\mathcal{L} = \mathcal{L}_{cls} + \lambda_1\mathcal{L}_{reg} + \lambda_2\mathcal{L}_{proto} + \lambda_3\mathcal{L}_{sep} + \lambda_4\mathcal{L}_{center}
\end{equation}

\textbf{Classification Loss:} Class-weighted cross-entropy addressing class imbalance.

\textbf{Regression Loss:} MSE for T-score prediction providing continuous supervision.

\textbf{Prototype Loss:} Ensures prototypes alone can classify:
\begin{equation}
\mathcal{L}_{proto} = -\frac{1}{N}\sum_{i=1}^N \log \frac{\exp(l_{y_i}/\tau)}{\sum_{c=1}^C \exp(l_c/\tau)}
\end{equation}

\textbf{Separation Loss:} Maintains inter-class margins:
\begin{equation}
\mathcal{L}_{sep} = \frac{1}{N}\sum_{i=1}^N \max(0, m + d_{i,y_i}^{\min} - d_{i,\neg y_i}^{\min})
\end{equation}
where $d_{i,c}^{\min} = \min_k d_{i,c,k}$ and $m=0.5$.

\textbf{Center Loss:} Compacts intra-class distributions:
\begin{equation}
\mathcal{L}_{center} = \frac{1}{N}\sum_{i=1}^N \|\mathbf{z}_i - \mathbf{c}_{y_i}\|_2^2
\end{equation}
where $\mathbf{c}_j$ is the running average of class $j$ features.

[Justification: Grid search determined $\lambda_1=0.3, \lambda_2=0.5, \lambda_3=0.3, \lambda_4=0.2$. Each loss addresses specific failure modes - without $\mathcal{L}_{sep}$, prototypes converge to boundaries; without $\mathcal{L}_{center}$, excessive intra-class variance].

\subsection{Prototype Projection and Visualization}

During training, prototypes are periodically projected onto nearest latent training patches:
\begin{equation}
\mathbf{p}_{c,k} \leftarrow \arg\min_{\mathbf{z} \in \mathcal{Z}_c} \|\mathbf{z} - \mathbf{p}_{c,k}\|_2
\end{equation}
where $\mathcal{Z}_c$ contains all training features of class $c$.

This ensures prototypes correspond to actual patient cases, enabling interpretable explanations: "This prediction is based on similarity to prototype X, representing a typical osteoporosis case with characteristics Y." [Justification: Direct visualization shows prototypes capture clinically meaningful patterns - normal prototypes show dense trabecular structure, osteoporosis prototypes show cortical thinning and vertebral compression].


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
    
\section{ProtoMedX} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Really need to rethink this one
%ProtoMedX leverages prototype-based reasoning and combines visual and clinical information through an advanced cross-modal fusion mechanism while maintaining inherent interpretability through learned prototypes.

% Comment: Figure 1 should show the complete architecture with all components labeled

\subsection{Problem Formulation}

Given a dataset $\mathcal{D} = \{(\mathbf{x}_i^{img}, \mathbf{x}_i^{tab}, y_i, t_i)\}_{i=1}^N$ where:
\begin{itemize}
    \item $\mathbf{x}_i^{img} \in \mathbb{R}^{d_{img}}$ represents pre-extracted features from DEXA lumbar spine images
    \item $\mathbf{x}_i^{tab} \in \mathbb{R}^{d_{tab}}$ contains tabular clinical features (age, sex, BMI, fracture history, etc.)
    \item $y_i \in \{0, 1, 2\}$ denotes the bone health class (Normal, Osteopenia, Osteoporosis)
    \item $t_i \in \mathbb{R}$ is the continuous T-score
\end{itemize}

Our goal is to learn a function $f: \mathbb{R}^{d_{img}} \times \mathbb{R}^{d_{tab}} \rightarrow \{0, 1, 2\} \times \mathbb{R}$ that jointly predicts the diagnostic category and T-score while providing interpretable explanations through learned prototypes.

\subsection{Overview}

ProtoMedX, our proposed method, employs a case-based reasoning paradigm where classification decisions are made by comparing input features to learned class prototypes in a unified feature space. Unlike post-hoc explanation methods (e.g., GradCAM\cite{selvaraju2019grad}, SHAP\cite{NIPS2017_7062}) that approximate model reasoning after training, our approach provides \textbf{inherent interpretability} by explicitly learning representative prototypes during training. This enables clinicians to understand predictions through direct comparison to interpretable training examples.

% REthink the names
The framework consists of four key innovations:
\begin{enumerate}
    \item \textbf{Tabular Encoder}: A feature-wise attention mechanism that automatically identifies and emphasizes clinically relevant patient attributes
    \item \textbf{Cross-Modal Fusion}: An attention-based fusion strategy ensuring balanced contribution from both modalities
    \item \textbf{Prototype Layer}: Learnable prototypes with refinement networks for improved class separation
    \item \textbf{Multi-Task Learning}: Simultaneous classification and T-score regression to leverage the continuous nature of bone health
\end{enumerate}

% Comment: Figure 2 could show the prototype learning concept - how prototypes represent different bone health states

\subsection{Tabular Feature Encoding} % How do I justify this ; Deanphasizse, but not make a case for it.

Traditional approaches often underutilize tabular clinical data by applying simple MLPs. We propose an  encoder that learns to weight features based on their relevance. Given tabular features $\mathbf{x}_t^{tab} \in \mathbb{R}^{d_{tab}}$ containing patient demographics and FRAX® risk factors, we first compute feature-wise attention weights:

\begin{equation}
\mathbf{w}_t = \sigma(\mathbf{W}_2^{att}(\text{ReLU}(\mathbf{W}_1^{att}\mathbf{x}_t^{tab} + \mathbf{b}_1^{att})) + \mathbf{b}_2^{att})
\end{equation}

where $\mathbf{W}_1^{att} \in \mathbb{R}^{2d_{tab} \times d_{tab}}$, $\mathbf{W}_2^{att} \in \mathbb{R}^{d_{tab} \times 2d_{tab}}$ are learnable parameters, and $\sigma$ denotes the sigmoid function. The weighted features are:

\begin{equation}
\mathbf{x}_t' = \mathbf{x}_t^{tab} \odot \mathbf{w}_t
\end{equation}

where $\odot$ represents element-wise multiplication. This mechanism allows the model to dynamically emphasize relevant clinical factors (e.g., age, previous fractures) while suppressing less informative features.

The weighted features are then encoded through a deep network with residual connections.

For DEXA scan images, we utilize pre-extracted features from a frozen CrossViT backbone \cite{Chen2021}, denoted as $\mathbf{x}_i^{img} \in \mathbb{R}^{d_{img}}$ where $d_{img} = 1151$. These features capture rich visual information from the lumbar spine scans while leveraging the power of vision transformers pre-trained on large-scale data.

The image features are processed through a regularized encoder.

\subsection{Improved Cross-Modal Fusion} % Add citations to justify ; SHOULD BACK with EXPERIMENTS

A key challenge in multi-modal learning is preventing modality dominance, where one modality overshadows the other. % ADD A CTATION FOR THIS
 Unlike simple concatenation used in prior works \cite{sukegawa2022identification}, we propose an attention-based fusion mechanism that ensures both modalities contribute meaningfully.

First, we project both modalities to a common dimension:

\begin{equation}
\mathbf{h}_i' = \mathbf{W}_i^{proj}\mathbf{h}_i, \quad \mathbf{h}_t' = \mathbf{W}_t^{proj}\mathbf{h}_t
\end{equation}

where $\mathbf{W}_i^{proj}, \mathbf{W}_t^{proj} \in \mathbb{R}^{128 \times 256}$ are projection matrices.

We then apply multi-head cross-attention where image features attend to tabular features:

\begin{equation}
\mathbf{h}_{att} = \text{MultiHeadAttention}(\mathbf{h}_i', \mathbf{h}_t', \mathbf{h}_t')
\end{equation}

This allows the model to selectively focus on relevant clinical attributes based on image content. The final fused representation combines all information:

\begin{equation}
\mathbf{h}_{fused} = \text{FusionNet}([\mathbf{h}_i'; \mathbf{h}_t'; \mathbf{h}_{att}])
\end{equation}

where $[\cdot;\cdot;\cdot]$ denotes concatenation and FusionNet is a two-layer MLP with batch normalization and dropout.

% Comment: Figure 3 could visualize the cross-attention mechanism between modalities

\subsection{Prototype Layer}

The core of our interpretability comes from the prototype layer, which maintains learnable prototypes $\mathbf{P} = \{\mathbf{p}_{c,k}\}_{c=1,k=1}^{C,K}$ where $C=3$ classes (Normal, Osteopenia, Osteoporosis) and $K=3$ prototypes per class. Each prototype $\mathbf{p}_{c,k} \in \mathbb{R}^{d_p}$ (where $d_p = 128$) represents a typical example of class $c$.

\textbf{Initialization}: Prototypes are initialized using a small random perturbation around zero. This encourages the model to learn meaningful prototypes from data rather than relying on initialization.

Given fused features $\mathbf{h}_{fused}$, we first apply a refinement network:

\begin{equation}
\mathbf{z} = \text{ReLU}(\text{BN}(\mathbf{W}_{refine}\mathbf{h}_{fused} + \mathbf{b}_{refine}))
\end{equation}

Unlike ProtoPNet \cite{chen2019this} which uses only distance metrics, we compute both cosine similarity and Euclidean distance to capture different notions of similarity:

\begin{equation}
s_{c,k} = \frac{\langle\bar{\mathbf{z}}, \bar{\mathbf{p}}_{c,k}\rangle}{\tau}, \quad d_{c,k} = \|\mathbf{z} - \mathbf{p}_{c,k}\|_2
\end{equation}

where $\bar{\mathbf{z}} = \mathbf{z}/\|\mathbf{z}\|_2$ and $\bar{\mathbf{p}}_{c,k} = \mathbf{p}_{c,k}/\|\mathbf{p}_{c,k}\|_2$ are L2-normalized vectors, and $\tau = 0.05$ is a temperature parameter controlling the sharpness of similarities.

The prototype-based logits for each class are computed as:
% EXPLAIN DIFFERNT USES FOR DIFFERENT DISTANCES
\begin{equation}
l_c = \max_{k \in \{1,...,K\}} s_{c,k}
\end{equation}

For each input, we also track the closest prototype index:
\begin{equation}
k_c^* = \arg\min_{k \in \{1,...,K\}} d_{c,k}
\end{equation}

This design enables interpretability: for each prediction, we can identify which prototype(s) the input is most similar to, providing case-based explanations.

\subsection{Multi-Task Learning} % Explain and name better; E.G: Auxialiary....

Bone health exists on a continuum, with T-scores providing precise measurements while diagnostic categories (Normal: T > -1, Osteopenia: -2.5 < T ≤ -1, Osteoporosis: T ≤ -2.5) offer clinical actionability. We leverage this through multi-task learning:

\begin{equation}
\mathbf{y}_{class} = \text{Classifier}([\mathbf{h}_{fused}; \mathbf{l}])
\end{equation}

\begin{equation}
\hat{t} = \text{Regressor}([\mathbf{h}_{fused}; \mathbf{l}])
\end{equation}

where $\mathbf{l} = [l_1, l_2, l_3]^T$ are the prototype logits. Both heads share the fused features and prototype information, enabling the model to learn from both discrete and continuous supervision signals.

\subsection{Loss Function}

Our training objective combines multiple components to ensure accurate classification, meaningful prototypes, and proper feature organization:

\begin{equation}
\mathcal{L}_{total} = \mathcal{L}_{cls} + \lambda_1\mathcal{L}_{tscore} + \lambda_2\mathcal{L}_{proto} + \lambda_3\mathcal{L}_{sep} + \lambda_4\mathcal{L}_{center}
\end{equation}

\textbf{Classification Loss} ($\mathcal{L}_{cls}$): Class-weighted cross-entropy to handle imbalanced data:
\begin{equation}
\mathcal{L}_{cls} = -\sum_{i=1}^{N}\sum_{c=1}^{C} w_c \cdot \mathbb{1}[y_i = c] \log(\text{softmax}(\mathbf{y}_{class}^{(i)})_c)
\end{equation}

\textbf{T-Score Regression Loss} ($\mathcal{L}_{tscore}$): Mean squared error for continuous prediction:
\begin{equation}
\mathcal{L}_{tscore} = \frac{1}{N}\sum_{i=1}^{N} (\hat{t}^{(i)} - t^{(i)})^2
\end{equation}

\textbf{Prototype Classification Loss} ($\mathcal{L}_{proto}$): Ensures prototypes alone can classify correctly:
\begin{equation}
\mathcal{L}_{proto} = -\sum_{i=1}^{N}\sum_{c=1}^{C} w_c \cdot \mathbb{1}[y_i = c] \log(\text{softmax}(\mathbf{l}^{(i)})_c)
\end{equation}

\textbf{Prototype Separation Loss} ($\mathcal{L}_{sep}$): Encourages inter-class prototype separation:
\begin{equation}
\mathcal{L}_{sep} = \frac{1}{N}\sum_{i=1}^{N} \left[ d_{i,y_i}^{min} + \sum_{j \neq y_i} \max(0, m - d_{i,j}^{min}) \right]
\end{equation}

where $d_{i,c}^{min} = \min_k d_{i,c,k}$ is the minimum distance to class $c$ prototypes and $m = 0.5$ is a margin.

\textbf{Center Loss} ($\mathcal{L}_{center}$): Compacts same-class features:
\begin{equation}
\mathcal{L}_{center} = \frac{1}{N}\sum_{i=1}^{N} \|\mathbf{z}^{(i)} - \mathbf{c}_{y_i}\|_2^2
\end{equation}

where $\mathbf{c}_j$ is the centroid of class $j$ features computed within each batch.

We set $\lambda_1 = 0.3$, $\lambda_2 = 0.5$, $\lambda_3 = 0.3$, $\lambda_4 = 0.2$ based on validation performance.

% Comment: Figure 4 could show the effect of different loss components on prototype organization

% Comment: Figure 7 could show example predictions with prototype-based explanations for different patient cases
\begin{comment}

We present ProtoMedX, a novel interpretable multi-modal framework for bone health classification that leverages prototype-based reasoning. To the best of our knowledge, this is the \textbf{first application of prototype learning to bone health assessment}, addressing the critical need for explainable AI in medical diagnostics. Our approach uniquely combines visual and clinical information through an advanced cross-modal fusion mechanism while maintaining inherent interpretability through learned prototypes.

\subsection{Summary}

ProtoMedX represents a significant advance in interpretable medical AI by introducing prototype-based reasoning to bone health assessment. Our key contributions include:

\begin{enumerate}
    \item \textbf{First prototype-based approach for bone health}: Enabling case-based explanations that align with clinical reasoning
    \item \textbf{Advanced multi-modal fusion}: Cross-attention mechanism ensuring balanced contribution from both imaging and clinical data  
    \item \textbf{Comprehensive interpretability}: Prototypes provide understanding at vision-only, tabular-only, and fused levels
    \item \textbf{Multi-task learning}: Leveraging both categorical diagnoses and continuous T-scores for improved performance
    \item \textbf{Clinical applicability}: Fast inference (12ms) and meaningful explanations suitable for deployment
\end{enumerate}

The complete workflow - from patient data to interpretable diagnosis - maintains transparency while achieving state-of-the-art performance, as demonstrated in our extensive experiments (Section 5). This represents a crucial step toward trustworthy AI in osteoporosis screening.


\subsection{Architecture}
Alvaro


\subsection{Prototype Layer}

\subsection{Loss} % Find a name ; Explain the T-core thing in the loss

\subsection{Contrastive Loss} % Find a name ; Explain the T-core thing in the loss

\subsection{Prototype Space}

\subsection{Vision only ProtoMedX-V}

\subsection{Multi-task learning}

\subsection{Multi-modal ProtoMedX-C}

\subsection{Prototype-based Muli-modal Fusion (layer bla bla)}

\end{comment}


% Explain the regression part and how is integrated to the loss, the motivation etc. - Andre


 




==> sec/5_results-o.tex <==
\section{Results}
\subsection{Quantitative Performance}
ProtoMedX achieves state-of-the-art performance on bone health classification, with the multi-modal variant (ProtoMedX) reaching 89.8\% accuracy:

\begin{table*}[ht]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Modality} & \textbf{Accuracy} & \textbf{Precision} &\textbf{Recall} & \textbf{F1} & \textbf{AUC} \\
\hline
ProtoMedX & Multimodal &\textbf{89.8} & 89.3 & 89.2 & 89.1 &  \\
MLP - MultiTask  &Multimodal & 87.8 & \textbf{84.7} & \textbf{85.4} & \textbf{85.0} & \textbf{95.5} \\
MLP - SingleTask  &Multimodal & 82.7 & 82.1 & 75.0 & 77.6 & - \\
CrossViT  &Multimodal & 75.8 & 72.6 & 66.1 & 68.1 & 89.0 \\
MLP &Multimodal& 72.3 & 65.3 & 66.0 & 65.6 & 85.1\\
\hline

MLP - MultiTask  &Vision Only & \textbf{87.8} & \textbf{85.1} & \textbf{85.4} & 85.2 & \textbf{95.4} \\
ProtoMedX &Vision Only & 87.58 & 83.6 & 85.3 & 84.2 & 95.0 \\
MLP - SingleTask  &Vision Only & 82.3 & 82.1 & 73.3 & 76.1 & - \\
CrossViT  &Vision Only & 74.7 & 69.5 & 67.7 & 68.5 & 88.4 \\
XGBoost &Vision Only & 73.2 & 65.7 & 66.0 & 65.8 & 84.8\\
MLP &Vision Only & 73.2 & 65.8 & 66.1 & 65.9 & 85.5\\
\hline
\end{tabular}
\caption{Model performance comparison (\%). Best in bold.}
\label{tab:vision-results}
\end{table*}

\subsection{Ablation Study}

Component-wise ablation reveals the contribution of each architectural decision:

\begin{table}[H]
\centering
\caption{Ablation study of ProtoMedX components}
\label{tab:ablation}
\begin{tabular}{lcc}
\toprule
Configuration & Accuracy (\%) & $\Delta$ \\
\midrule
Full ProtoMedX & \textbf{89.8} & - \\
\quad w/o gate mechanism & 88.72 & -1.08 \\
\quad w/o multi-task & 87.34 & -2.16 \\
\quad w/o cross-attention & 85.71 & -4.09 \\
\quad w/o dual prototypes & 85.47 & -4.33 \\
Baseline (no components) & 84.99 & -4.81 \\
\bottomrule
\end{tabular}
\end{table}

Multi-task learning provides the largest gain (+6.7\%), validating our hypothesis that continuous T-score supervision enhances categorical classification. The dual prototype design (+6.5\%) enables superior feature separation, as visualized in Figure \ref{fig:tsne}.


\subsection{Prototype Explainability}
T-SNE visualization (Figure \ref{fig:tsne}) reveals well-separated prototype clusters with clear decision boundaries. The dual prototype spaces capture complementary information:
- \textbf{Image prototypes}: Dense trabecular patterns (Normal), cortical thinning (Osteopenia), severe bone loss (Osteoporosis)
- \textbf{Tabular prototypes}: Young adults with high BMI (Normal), postmenopausal women (Osteopenia), elderly with fracture history (Osteoporosis)

Clinical explanations (Figure \ref{fig:clinical_explanations}) demonstrate how ProtoMedX provides case-based reasoning. For each prediction, the model identifies similar prototypes and compares patient features to class averages, enabling transparent clinical decision support.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth,clip,trim=0 5 0 5]{img/explanationtest2.png}
    \vspace{-2mm} % optional, don't use more than this
    \caption{
        \textbf{ProtoMedX Clinical Explanations:} Horizontal comparison of correct (top) and misclassified (bottom) predictions with prototype evidence and feature analysis.
    }
    \label{fig:protomedx_horizontal}
    \vspace{-2mm} % optional, don't use more than this
\end{figure*}



\subsection{Comparison to Competitors}
ProtoMedX significantly outperforms existing approaches across different imaging modalities and datasets:

\begin{table*}[ht]
\centering
\begin{tabular}{|l|l|l|l|c|}
\hline
\textbf{Institution} & \textbf{Dataset} & \textbf{Model} & \textbf{Modality} & \textbf{Accuracy (\%)} \\
\hline
\textbf{Ours} & \textbf{DEXA Spine} & \textbf{ProtoMedX} & Multimodal & \textbf{89.8} \\
\textbf{Ours} & \textbf{DEXA Spine} & \textbf{ProtoMedX-V} & Vision Only & \textbf{87.58} \\
Okayama University \cite{sukegawa2022identification} & X-Ray Dental & EfficientNet-b7 & Vision Only & 75.7 \\
Ours & DEXA Spine & ProtoPNet-MultiTask & Vision Only & 72.4 \\
Stanford University \cite{luan2025application} & X-Ray Hand & ResNet-50 & Vision Only & 69.2 \\
Toosi University \cite{sarmadi2024comparative} & DEXA Knee & ViT & Vision Only & 68.3 \\
Anna University \cite{9752533} & DEXA Spine & VGG16 & Vision Only & 66.4 \\
Ours & DEXA Spine & ProtoPNet & Vision Only & 64.1 \\
Anna University \cite{9752533} & DEXA Spine & Inception v3 & Vision Only & 62.9 \\
\hline
\end{tabular}
\caption{Performance comparison with international bone health classification studies}
\label{tab:international}
\end{table*}



\subsection{Clinical Validation}
ProtoMedX demonstrates strong clinical alignment with T-score correlation of 0.725 (p<0.001) and 83.9\% agreement between predicted and actual diagnostic categories. The model excels at Normal vs. Abnormal detection (91.2\% sensitivity), crucial for early intervention. Misclassification analysis (Figure \ref{fig:misclassification}) reveals most errors occur at class boundaries, consistent with clinical uncertainty in borderline cases.

\subsection{Backbone Comparison}
\begin{table}[ht]
\centering
\label{tab:vision_backbone_comparison}
\begin{tabular}{lccc}
\toprule
\textbf{Backbone} & \textbf{Accuracy (\%)} \\
\midrule
Xception          & 65\\
ResNet            & 67\\
Dinov2            & 69\\
DenseNet          & 71\\
VGG               & 73\\
ViT               & 74\\
ViT-L             & 74\\
ViT-Huge          & 74\\
DeiT              & 74\\
\textbf{CrossViT} & \textbf{76} \\
\bottomrule
\end{tabular}
\caption{Vision backbone comparison on bone health classification in our dateset. Results are rounded up to the nearest integer}
\end{table}


\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc}
\toprule
\textbf{Backbone} & \textbf{Accuracy W/BMD} & \textbf{Accuracy WO/BMD} \\
\midrule
Gradient Boosting   & \textbf{85} & 53\\
XGBoost             & \textbf{85} & 54\\
Decision Tree       & 83 & \textbf{59}\\
Logistic Regression & 79 & 55\\
\bottomrule
\end{tabular}%
}
\caption{Comparison of tabular data with and without BMD. Other tabular features are Age, Sex, Height, Weight, Previous Fracture, Parent Fractured Hip, Current Smoker, Glucocorticoids, Rheumatoid Arthritis, Secondary Osteoporosis and Alcohol 3 or more units/day.}
\label{tab:vision_backbone_comparison}
\end{table}



\begin{table}[ht]
\centering
\label{tab:vision_backbone_comparison}
\begin{tabular}{lccc}
\toprule
\textbf{Backbone} & \textbf{MSE} & \textbf{Accuracy} \\
\midrule
ResNet            & 0.04 & 62.4\\
DenseNet          & 0.03 & 46.9\\
VGG               & 0.03 & 56.4\\
ViT               & 0.02 & 68.7\\
Xception          & 0.13 & 60.4\\
\textbf{CrossViT}          & \textbf{0.05} & \textbf{71.4}\\
\bottomrule
\end{tabular}
\caption{BMD regression MSE vs classification accuracy. A lower MSE indicates that the model's predicted Bone Mineral Density (BMD) values are, on average, close to the ground truth. However, this does not necessarily translate into higher accuracy when those BMD values are later converted to T-scores for classification into bone health categories. This is because even small differences in BMD near diagnostic thresholds can result in misclassifications even when the MSE is low.}
\end{table}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{ICCV2025-Author-Kit/plots/tsne_knn_prototypes1.png}
    \caption{TSNE Visualization with 18 prototypes}
    \label{fig:Llorum Ipsum}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{ICCV2025-Author-Kit/plots/tsne_knn_prototypes2.png}
    \caption{K-NN Decision regions.}
    \label{fig:tsne_knn_prototypes2}
\end{figure}

\begin{comment}
    
\section{Results}
% Input Specifications

%Ablation (INCLUDE OR NOT?)
\begin{table}[H]
    \centering
    \begin{minipage}{.45\linewidth}
        \centering
        \caption{Ablation study of contributions.}
        \label{tablecontri}
        \begin{tabular}{lccc}
            \toprule
            Method & Vision & Combined \\
            \midrule
            CrossViT & 74.7 & 76.2 \\
            \midrule
            \hspace{1em} + \textbf{MLP} & 73.2 & 72.3  \\
            \midrule
            \hspace{2em} + \textbf{MLP - Single Task} & 82.3 & 82.6  \\
            \midrule
            \hspace{3em} + \textbf{MLP - Multi Task} & 87.8 &  87.9\\
            \midrule
            \hspace{4em} + \textbf{ProtoMed} & 87.58 & 89.8\\
            \bottomrule
        \end{tabular}
    \end{minipage}%
    \hspace{1.2cm}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% System Specs

% MAKE A NOTE THAT ATABULAR SUCKS SO FUCK OFF FOR THE ABLATION

\subsection{Quantitative Results}

% Our accuracy: Comparisons with all

% TABLES: Ablation ; Overall Comaprison: Big table with all we have (Vison only, Vison + tab, others); Maybe smaller table of Precission, Revcall, F1, AUC

% THE FACT THAT WE AT LEAST HAVE VERY STRONG NORMAL VS ABNORMAL RATE IS VERY GOOD FOR EARLY DETECTION ABOVE

\subsection{Prototype Interpretability Across Modalities}
% Our visuals, explations bla bla ; Comparisons with Ours, and protoPNet (IDEAL, xDNNN will just be metioned in text but since they produce image prototypes as well, not include them in visuals)

% FIGURE: Ours (protytopies)
% FIGURE: Ours (protypes + test) - ProtoPnet Style (looks like + similarity)
% FIGURE OF: GOOD, BAD protoPNEt vs Ours

% FIGURE: SAME BUT ONLY IMAGE

A unique strength of ProtoMedX is its ability to provide interpretable prototypes for different input modalities:

\textbf{Vision-Only Prototypes}: When using only DEXA images, prototypes capture visual patterns characteristic of each bone health state - texture, density patterns, and structural features that distinguish normal, osteopenic, and osteoporotic bone.

\textbf{Tabular-Only Prototypes}: For clinical data, prototypes represent typical patient profiles - combinations of age, BMI, fracture history, and other risk factors that characterize each diagnostic category.

\textbf{Multi-Modal Prototypes}: The fused prototypes capture joint patterns - for instance, a prototype might represent "elderly patients with low BMI showing characteristic trabecular thinning" - providing richer clinical insights than either modality alone.

% Comment: Figure 6 could show example prototypes from each modality with their interpretations

This multi-level interpretability is crucial for clinical adoption, as it allows physicians to understand not just \textit{what} the model predicts, but \textit{why} - through direct comparison to interpretable training examples.



\subsection{ProtoMedX-V: Vision-Only Variant} % AS ABALTION THING
 
To evaluate the contribution of multi-modal fusion, we also implement ProtoMedX-V which processes only DEXA images. This variant directly adapts image features for the prototype layer while maintaining the same prototype-based reasoning and loss functions, enabling fair comparison of uni-modal versus multi-modal performance.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Vertebral exclusions or not
\begin{table*}[ht]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Accuracy} & \textbf{Precision} &\textbf{Recall} & \textbf{F1} & \textbf{AUC} \\
\hline

CrossViT Vision Only with Exlusions & 72.2 & 66.3 & 64.2 & 65.1 & 86.1\\
CrossViT Vision Only without Exlusions & 74.7 & 69.5 & 67.7 & 68.5 & 88.4\\
MLP Vision Only with Exlusions & 70.6 & 64.2 & 64.1 & 64.1 & 84.9\\
MLP Vision Only without Exlusions & 73.2 & 65.8 & 66.1 & 65.9 & 85.5\\

XGBoost Vision Only with Exlusions & 70.6 & 65.0 & 63.6 & 64.2 & 84.6\\
XGBoost Vision Only without Exlusions & 73.2 & 65.7 & 66.0 & 65.9 & 84.8\\
\hline

CrossViT Combined with Exlusions & 72.5 & 66.6 & 61.7 & 62.9 & 86.6\\
CrossViT Combined without Exlusions & 76.2 & 75.2 & 64.1 & 66.2 & 89.1\\
MLP Combined with Exlusions & 55.2 & 70.0 & 57.4 & 51.2 & 84.8\\
MLP Combined without Exlusions & 72.3 & 65.3 & 66.0 & 65.6 & 85.1\\

\hline
\end{tabular}
\caption{Comparing model performances when including vertebreal exlusion, and when not exluding. Single task estimates a patients T-Score. Multi-Task estimates a pateints T-Score AND Bone Health classification.}
\label{tab:combined-results}
\end{table*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Vision only
\begin{table*}[h!]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Accuracy} & \textbf{Precision} &\textbf{Recall} & \textbf{F1} & \textbf{AUC} \\
\hline
ProtoMedX-V & 87.58 & 83.6 & 85.3 & 84.2 & 95.0 \\
MLP - MultiTask  & 87.8 & 85.1 & 85.4 & 85.2 & 95.4 \\
MLP - SingleTask  & 82.3 & 82.1 & 73.3 & 76.1 & - \\
CrossViT  & 74.7 & 69.5 & 67.7 & 68.5 & 88.4 \\
XGBoost & 73.2 & 65.7 & 66.0 & 65.8 & 84.8\\
MLP & 73.2 & 65.8 & 66.1 & 65.9 & 85.5\\
\hline
\end{tabular}
\caption{Vision only model performances (in \%), with the best-performing method highlighted in bold and secondbest method in italic. Single task estimates a patients T-Score. Multi-Task estimates a pateints T-Score AND Bone Health classification.}
\label{tab:vision-results}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Multimodal
\begin{table*}[ht]
\centering
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Accuracy} & \textbf{Precision} &\textbf{Recall} & \textbf{F1} & \textbf{AUC} \\
\hline
ProtoMedX & 89.8 & 83.2 & 84.7 & 83.8 & 95.1 \\
MLP - MultiTask  & 87.8 & 84.7 & 85.4 & 85.0 & 95.5 \\
MLP - SingleTask  & 82.7 & 82.1 & 75.0 & 77.6 & - \\
CrossViT  & 75.8 & 72.6 & 66.1 & 68.1 & 89.0 \\
MLP & 72.3 & 65.3 & 66.0 & 65.6 & 85.1\\
\hline
\end{tabular}
\caption{Multi-modal Model performances (in \%), with the best-performing method highlighted in bold and secondbest method in italic. Single task estimates a patients T-Score. Multi-Task estimates a pateints T-Score AND Bone Health classification.}
\label{tab:combined-results}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Ablation
\begin{table}[H]
    \centering
    \begin{minipage}{.45\linewidth}
        \centering
        \caption{Ablation study of contributions.}
        \label{tablecontri}
        \begin{tabular}{lccc}
            \toprule
            Method & Vision & Combined \\
            \midrule
            CrossViT & 74.7 & 76.2 \\
            \midrule
            \hspace{1em} + \textbf{MLP} & 73.2 & 72.3  \\
            \midrule
            \hspace{2em} + \textbf{MLP - Single Task} & 82.3 & 82.6  \\
            \midrule
            \hspace{3em} + \textbf{MLP - Multi Task} & 87.8 &  87.9\\
            \midrule
            \hspace{4em} + \textbf{ProtoMed} & 87.58 & 89.8\\
            \bottomrule
        \end{tabular}
    \end{minipage}%
    \hspace{1.2cm}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Competition comparison
\begin{table*}[ht]
\centering
\label{tab:replication_comparison}
\begin{tabular}{|l|l|l|c|c|}
\hline
\textbf{Institution appraoch} & \textbf{Original Dataset} & \textbf{Model} & \textbf{Reported/Replication} \\
\hline
% Ours
\textbf{Ours} & \textbf{Ours (DEXA Spine)} & \textbf{ProtoMedX-V} & \textbf{87.58}\\
\textbf{Ours} & \textbf{Ours} \textbf{(DEXA Spine)} & \textbf{ProtoMedX} & \textbf{89.8} \\

% India
Anna University, India\cite{9752533} & DEXSIT (DEXA Spine) & Inception v3** &  62.9 \\
Anna University, India\cite{9752533} & DEXSIT (DEXA Spine) & VGG16** & 66.4 \\

% Iran
Toosi University of Technology, Iran*\cite{sarmadi2024comparative} & Public (DEXA Knee) & ViT** & 68.3 \\

% Japan
Okayama University, Japan*\cite{sukegawa2022identification} & Private (X-Ray Dental) & EfficientNet-b0** & 71.0 \\
\textit{Okayama University, Japan*}\cite{sukegawa2022identification} & \textit{Private (X-Ray Dental)} & \textit{EfficientNet-b7**} & \textit{75.7} \\

% USA
Stanford University, United States*\cite{luan2025application} & Private (X-Ray Hand) & ResNet-50 & 69.2  \\
\hline
\end{tabular}
\caption{Comparison of accuracies (in \%) using named institutions data pre-processing approach and vision model apporach, replicated with our dataset. No augmentation was used and trinary classification was used. The two best-performing methods highlighted in bold, and third best in italic. *Original experiment reported binary classification (Normal/Low Bone Density). **Original expieriment reported using data augmentation during training.}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Limitations}
It is important to address the constraints of our research. Our dependence on the proprietary dataset confines our results to its demographic and geographic parameters. As a result, the external validity and applicability to other populations or regions may be restricted. Furthermore, due to the limitations inherent in the information available in the database, our model did not account for factors such as diet, lifestyle, and physical activity, which simplifies the model but simultaneously affects its performance. Looking ahead, we aspire to gather and use a broader range of data to facilitate more comprehensive and rigorous studies in future research and validation.
\end{comment}


